MuxServe: Flexible Spatial-Temporal Multiplexing for Multiple LLM Serving

Large language models (LLMs) have demonstrated remarkable performance, and organizations are racing to serve LLMs of varying sizes as endpoints for use-cases like chat, programming and search. However, efficiently serving multiple LLMs poses significant challenges for existing approaches due to varying popularity of LLMs. In the paper, we present MuxServe, a flexible spatial-temporal multiplexing system for efficient multiple LLM serving. The key insight behind is to colocate LLMs considering their popularity to multiplex memory resources, and leverage the characteristics of prefill and decoding phases to separate and flexibly colocate them to multiplex computation resources. MuxServe formally formulates the multiplexing problem, and proposes a novel placement algorithm and adaptive batch scheduling strategy to identify optimal colocations and maximize utilization. MuxServe designs a unified resource manager to enable flexible and efficient multiplexing. Evaluation results show that MuxServe can achieves up to $1.8\times$ higher throughput or processes $2.9\times$ more requests within $99\%$ SLO attainment. The code is available at: \url{https://github.com/hao-ai-lab/MuxServe}.

==> tex/old_method.tex <==
\section{Method}

\subsection{Problem Formulation}
Consider we have a cluster $C$ and a set of LLMs $M$ to be served, one key insight \Sys leveraged to improve system utilization is to colocate LLMs considering their popularity. LLMs with high request rates can be colocated together with LLMs with low request rates to efficiently utilize resources. To achieve this, we introduce \textit{LLM bundle}, which refers to a group of LLMs that will be colocated together with the GPUs they are assigned to. Our goal is to find the best \textit{LLM bundles} $B^*$ that can maximize GPU utilization (i.e. throughput), hence the problem can be formulated as,

% \Sys groups them into \textit{LLM bundles} for efficient multiplexing. A \textit{LLM bundle} encompasses a group of LLMs that will be colocated together with the GPUs they are assigned to. Our goal is to find the best \textit{LLM bundles} $B^*$ that can maximize GPU utilization, hence the problem can be formulated as,

\begin{equation}
\begin{aligned}
\label{eq:inter_bundle}
   B^* = \argmax_{B\in \mathcal{B}} \sum_{b\in B} \texttt{tpt}(b)
\end{aligned}
\end{equation}

where $\mathcal{B}$ represents all possible LLM bundles candidate, and \texttt{tpt}($\cdot$) estimates the throughput for a LLM bundle $b$. 

Within a LLM bundle, \Sys exploits the characteristics of prefill and decoding phases, separates them to different jobs, and flexibly colocates them to multiplex resources.
However, as there are multiple LLMs with distinct popularity and request length distribution, different batching and scheduling strategies of these LLMs can lead to different throughputs, and different LLMs may also compete for resources. Therefore, given a LLM bundle $b$, we need to find the optimal strategy $S$ that can maximize the throughput while ensuring fair sharing among LLMs, 

\begin{equation}
\begin{aligned}
\label{eq:intra_bundle}
    \texttt{tpt}(b) = \max_{S} \sum_{m \in b_{llm}} \texttt{throughput}_S(m, b) \\
    s.t. \quad \forall m_i, m_j \in b_{llm}, \quad |\texttt{R}(m_i) - \texttt{R}(m_j)| \le \epsilon
\end{aligned}
\end{equation}

where $\texttt{throughput}_S$($\cdot$, $\cdot$) estimates the throughput of a LLM in a bundle with $S$, \texttt{R}($\cdot$) represents the resources a LLM use, and $\epsilon$ is a small number that controls fairness. 

Given the formulation above, we first present our batching and scheduling strategy to maximize the throughput within a LLM bundle (\Cref{eq:intra_bundle}) in \Cref{method:adbs}. Finally we introduce our placement algorithm to solve the problem (\Cref{eq:inter_bundle}) in \Cref{method:place}.

\subsection{Batching and Scheduling}
\label{method:adbs}

% The cluster is divided into several group of devices, with each group assigned to serve a specific subset of LLMs using intra-operator parallelism. The primary objective is to find the group of LLM bundles that maximizes the cluster utilization, i.e. the serving throughput. 

% Consider we have a cluster $C$ and a group of LLMs $M$ to be served. The workload 

\JF{==== Bellowing is old method =====}

In this section, we first introduce our resource manager to enable efficient multiplexing in \Cref{method:res_manager}. Then we describe \textit{adaptive batch scheduling} mechanism to ensure fairness and prevent starvation in \Cref{method:fairness}. Finally we present our placement algorithm to determine how to collocate LLMs in \Cref{method:place}.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/arch.pdf}
  \caption{Overview of GPU resource management in a LLM bundle, which represents a group of LLMs and GPUs.}
  \label{fig:arch}
\end{figure}

\subsection{Resource Management}
\label{method:res_manager}

As discussed in \Cref{bg:opportunity}, the spatial-temporal multiplexing of LLMs faces challenges in both computation and memory aspects. First, the \textit{prefill} and \textit{decoding} phases exhibit distinct computation resources requirements. Second, memory becomes a critical bottleneck when collocating LLMs, since each LLM necessitates a substantial space for model weight and KV cache. Consequently, \Sys needs to design mechanisms for GPU resources sharing to enable efficient spatial-temporal multiplexing of multiple LLMs. 

\Sys divides the GPU cluster and LLMs to be served into \textit{LLM bundles}. A \textit{LLM bundle} encompasses a group of LLMs that will be colocated together with the GPUs they are assigned to. \Cref{fig:arch} shows the overview of GPU resource management in a LLM bundle, which is the basic unit in \Sys. The computation and memory resources in a LLM bundle are managed in different strategies.


The computation resources in a LLM bundle are shared in units of SM (Streaming Multiprocessor). Each GPU contains a fixed number of SM resources. These SMs can be dynamically allocated to different tasks during runtime rather than being statically assigned to a single job. \Sys decouples the two phases of LLM inference into \textit{prefill} and \textit{decoding} jobs, and assigns SM resources to them separately. During serving, the LLM bundle schedules jobs from different LLMs to the parallel runtime, as long as the SM resources requirements of jobs do not exceed the GPU limit. This flexible sharing of SM resources allows for efficient utilization and enables concurrent execution of inference jobs within a LLM bunde.

The memory consumption of LLM serving mainly consists of three parts: model weight, activation and KV cache. In single LLM serving, the whole memory space is occupied exclusively by one job. To serve multiple LLMs concurrently, one prominent challenge lies in sharing the memory space among different jobs to reduce memory waste and fragmentation. To tackle this challenge, \Sys organizes and manages the GPU memory within a LLM bundle as a unified memory space, which is divided into three distinct partitions, each dedicated to storing different types of model data. 

The first partition stores a single replica of model weights for each LLM in the bundle. This design reduces redundancy, as both the \textit{prefill} and \textit{decoding} jobs of a particular LLM require the same model weights for computation. During serving, different jobs within the LLM bundle can seamlessly access and utilize these shared model weights.

The second partition reserves space for activation, which is utilized during inference runtime. LLM inference requires additional memory to store intermediate results (activations). Notably, \textit{prefill} jobs typically demand a significant amount of extra memory. When collocating multiple LLMs, reserving additional memory for each job results in substantial memory waste, as the number of jobs that can be executed concurrently is limited. Consequently, \Sys adopts a shared activation space to reduce waste.

The final partition serves as a unified KV cache space, which accommodates the KV cache of different LLMs. The KV cache is known to consume a huge amount of memory and has a considerable impact on the throughput of LLM inference. However, the allocation of KV cache memory poses challenges. Dynamic on-demand allocation can lead to significant memory fragmentation~\cite{vllm}. Conversely, static allocation for each LLM disregards the varying arrival rates of LLMs. This results in popular LLMs being unable to utilize the KV cache space of less popular LLMs, which could otherwise enhance serving throughput.

To address this issue, \Sys introduces a unified KV cache space for LLM multiplexing. To enable efficient sharing of the unified KV cache among various LLMs, \Sys proposes head-wise cache, which holds the KV cache for a single head of a token. The unified KV cache space is divided into numerous head-wise cache blocks and allocated in fine granularity. This approach is based on the observation that although different LLMs possess varying numbers of attention heads, hidden layers, and hidden sizes, the size of each attention head is often consistent or has limited variations across different LLMs. Leveraging this observation, \Sys allocates KV cache in units of attention heads and hidden layers as illustrated in \Cref{fig:arch}. This allows for efficient sharing and utilization of cache resources across jobs while accommodating the specific architectural characteristics of LLMs. In addition, we also implement custom head-wise attention kernels based on PagedAttention~\cite{vllm}.

By consolidating the memory into a unified space and partitioning computation resources flexibly during runtime, the LLM bundle optimizes memory utilization and facilitates seamless sharing of resources among different jobs, thus enabling efficient spatial-temporal multiplexing of different inference jobs.


\begin{algorithm}[t]
   \caption{Adaptive Batch Scheduling (ADBS)}
   \label{alg:adbs}
\begin{algorithmic}
   \STATE {\bfseries Input:} LLM list $M$
   \STATE $prefill\_waiting$ $\leftarrow$ false
   \WHILE{True}
   \IF{no prefill jobs in execution}
   \STATE $m \leftarrow$ select a prefill job with round-robin from $M$
   \IF{resource is enough for $m$}
   \STATE schedule $m$ to execute
   \STATE $prefill\_waiting \leftarrow$ False
   \ELSE
   \STATE $prefill\_waiting \leftarrow$ True
   \ENDIF
   \ENDIF

    \IF{not $prefill\_waiting$}
    \WHILE{resource is enough}
    \STATE schedule a decoding job with round-robin
    \ENDWHILE
    \ENDIF
    \ENDWHILE
\end{algorithmic}
\end{algorithm}

\subsection{Batching and Scheduling}
\label{method:fairness}

The batching and scheduling of single LLM serving has been extensively studied. Iteration-level batching~\cite{orca} and first-come-first-serve (FCFS) scheduling~\cite{vllm} are widely adopted approaches to prevent starvation and ensure fairness. With these approaches, the earliest arrived requests are served first and requests are batched in fine-grained iteration level instead of request level to enhance performance.

However, when it comes to multiplexing multiple LLMs, these approaches encounter challenges due to the diverse workload characteristics among LLMs within a bundle, including variations in arrival rates and request length distributions. Moreover, requests for different LLMs cannot be batched together due to distinct model architectures and shapes. To tackle these challenges, we propose \textit{adaptive batch scheduling} (ADBS) to dynamically adjust the batching and scheduling of LLMs within the bundle during runtime, ensuring fair sharing of resources and preventing starvation.

% batching: iteration-level, limit batch size
Based on the observation that KV cache size poses a significant performance bottleneck in LLM serving, \Sys takes a proactive approach by dynamically adapting the KV cache sizes for each LLM to ensure fair sharing. Since the token KV cache size varies among LLMs, allowing them to utilize an equal amount of KV cache blocks could result in differing numbers of tokens. Therefore, \Sys prioritizes fairness by considering token counts. Additionally, to account for variations in arrival rates, \Sys further adjusts the number of tokens that each LLM can hold in the KV cache based on the ratio of their respective rates. At runtime, \Sys batches requests separately for each LLM with iteration-level batching~\cite{orca} and continuously monitors the KV cache utilization of each LLM periodically. With these monitoring statistics, \Sys identifies low-utilization LLMs and proactively transfers KV cache blocks from these LLMs to high-utilization LLMs. This dynamic reallocation of KV cache blocks ensures optimal utilization of resources and promotes efficient sharing among the LLMs within a bundle.

% \Sys also incorporates a redistribution mechanism help enhance overall efficiency. 

% scheduling: round-robin
\Sys explores two types of collocations to improve utilization: \textit{prefill-decoding} and \textit{decoding-decoding} collocation. This is motivated by the observation that \textit{prefill} phases typically requires a large amount of computation resources. \Cref{alg:adbs} describes the scheduling of ADBS. \Sys prioritizes prefill jobs to maximize utilization and adopts a round-robin approach to schedule LLMs within the bundle. \Sys continues scheduling decoding jobs for execution unless there is a prefill task waiting for resources. 


\begin{algorithm}[t]
   \caption{Enumeration-based Greedy Model Placement}
   \label{alg:placement}
\begin{algorithmic}
   \STATE {\bfseries Input:} LLM list $M$, cluster $C$, workload $W$
   \STATE {\bfseries Output:} The group of LLM bundle $best\_bundles$
   \STATE $\hat{M} \leftarrow$ get\_partition\_candidate($M$, $W$)
   \STATE $\mathcal{D} \leftarrow$ get\_potential\_device\_meshes($C$, $M$)

   \STATE $best\_tpt, best\_bundles \leftarrow 0, None$
   \FOR{$D \in \mathcal{D}$}
   % \STATE $bundles, tpt \leftarrow$ ILP\_bundle\_opt($\hat{M}$, $D$)
   \STATE // Greedily place LLMs on mesh group $D$
   \STATE $M'$=sort($\hat{M}$, $key$=$computation$, $ascend$=$False$)
   \FOR{$m \in M'$}
   \STATE $best\_mesh, max\_delta$ $\leftarrow$ None, -1
   \FOR{$d \in D$}
   \STATE $delta$ = estimate\_throughput\_increase($m$, $d$)
   \IF{$delta > max\_delta$}
   \STATE $best\_mesh, max\_delta$ = $d, delta$
   \ENDIF
   \ENDFOR
   \STATE $best\_mesh$.place($m$)
   \ENDFOR

   \STATE $tpt$ = estimate\_throughput($M', D$)
   \IF{$best\_tpt < tpt$}
   \STATE $best\_tpt, best\_bundles \leftarrow tpt, (M', D)$
   \ENDIF
   \ENDFOR
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
   \caption{Model Partition Candidate Generation}
   \label{alg:candidate}
\begin{algorithmic}
   \STATE {\bfseries Input:} LLM list $M$, workload $W$
   \STATE {\bfseries Output:} The parition candidate $\hat{M}$
   \STATE $\hat{M} \leftarrow []$
   \FOR{$m \in M$}
   \STATE $sm\_list \leftarrow$ get\_potential\_sm\_list($m$)
   \STATE $tp\_list \leftarrow$ get\_potential\_tp\_degree($m$)
   \FOR{$p \in tp\_list$}
   \FOR{$num\_sm \in$ sorted($sm\_list$)}
   \STATE $tpt, bs \leftarrow$ estimate\_throughput($m, num\_sm, p$)
   \IF{$tpt \ge W$.get\_rate($m$)}
   \STATE $m$.add\_candidate(($p, num\_sm, bs$))
   \STATE {\bfseries break}
   \ENDIF
   \ENDFOR
   \ENDFOR
   \STATE $\hat{M}$.append($model\_dandidate$)
   \ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Placement Algorithm}
\label{method:place}

Given a set of LLMs and a fixed cluster, \Sys groups them into LLM bundles for efficient multiplexing. The cluster is divided into several group of devices, with each group assigned to serve a specific subset of LLMs using intra-operator parallelism. The primary objective is to find the group of LLM bundles that maximizes the cluster utilization, i.e. the serving throughput. 

However, determining the optimal group of LLM bundles poses a challenging combinatorial optimization problem. As the number of devices and models increases, the total number of possible LLM bundle combinations grows exponentially. To solve this optimization problem, we design a two-level algorithm. As described in \Cref{alg:placement}, \Sys first enumerates potential device mesh groups. Each mesh comprises several GPUs that will be used to serve a set of LLMs concurrently. Then \Sys greedily places LLMs on a given device mesh group. \Sys selects the group of LLM bundles that achieve the highest estimated serving throughput as the serving configuration.

In \Cref{alg:placement}, \Sys first generates all possible model partition candidates $\hat{M}$ considering the workload $W$. \Cref{alg:candidate} shows the pseudo-code to generate candidates. For each LLM $m$, \Sys enumerates all possible configuration combinations of number of SMs and intra-operator parallelism degree. \Sys estimates throughput for each configuration, and selects the configuration that requires minimum number of SMs for each intra-operator parallelism degree as possible partition candidate. 

\Sys then enumerates all potential device mesh groups to find the optimal LLM bundles. Given a device mesh group $D$ and a list of model partition candidates $\hat{M}$, \Sys greedily place LLMs on meshes to find the group of LLM bundles that can maximize throughput. Since the target is to maximize serving throughput, \Sys first sorts LLMs in descending order according to arrival rates and prioritizes the placement selection for LLMs with high arrival rates. For a specified LLM $m$, \Sys iterates over all available meshes and approximates the expected increase in throughput with \texttt{estimate\_throughput\_increase}. The LLM $m$ is then placed on the mesh that yields the maximum throughput increase. This process is repeated for all LLMs. Subsequently, \Sys utilizes the \texttt{estimate\_throughput} function to estimate the serving throughput of the LLM bundles after the placement. Finally, \Sys selects the LLM bundles that offer the best serving throughput as the optimal serving configuration.


\paragraph{Throughput Estimator.} 
In order to estimate the serving throughput of LLM in a bundle, \Sys builds a simple yet effective analytical estimator with the following formula to estimate the throughput of LLM $i$,

\begin{equation}
    p_i = \frac{b^{i}}{\sum_{m\in bundle}t^{m}_{p} + t^{i}_{d} \times l^{i}_{o}}
\end{equation}

where $t_{p}, t_{d}$ and $l_{o}$ represent the prefill latency, decoding latency and average generation length of a batch requests with size $b$, respectively. The average generation length can be estimated from requests history or specific dataset, ShareGPT~\cite{sharegpt} for instance. The prefill and decoding latency of different batches and request length can be profiled in advance. This formula is based on the observation that prefill phases are executed sequentially and decoding phases can be executed concurrently. Given the request arrival rates, we can use binary search to find the batch size $b$ that can satisfy the traffic. 

% Given a LLM request arrival rate, we can use binary search to find the batch size $B$ that can satisfy the traffic. 


% For single LLM serving, \Sys estimates the throughput with the following equation,
% \begin{equation}
%     TPT = \frac{B}{t_{prefill} + t_{decoding} \times l_{output}}
% \end{equation}
% where $t_{prefill}, t_{decoding}$ and $l_{output}$ represent the prefill latency, decoding latency and average generation length of a batch requests with size $B$, respectively. The average generation length can be estimated from requests history or specific dataset, ShareGPT~\cite{sharegpt} for instance. The prefill and decoding latency of different batches and request length can be profiled in advance. Given a LLM request arrival rate, we can use binary search to find the batch size $B$ that can satisfy the traffic. 

% In order to estimate the serving throughput of LLM in a bundle, \Sys extends the previous equation to estimate the throughput of LLM $i$ with,

% \begin{equation}
%     TPT_i = \frac{B^{i}}{\sum_{m\in bundle}t^{m}_{prefill} + t^{i}_{decoding} \times l^{i}_{output}}
% \end{equation}

% This is based on the observation that prefill phases are executed sequentially and decoding phases can be executed concurrently.


==> tex/old_placement.tex <==
\subsection{Placement Algorithm}
\label{method:place}

Given a set of LLMs and a fixed cluster, \Sys groups them into LLM bundles for efficient multiplexing. The cluster is divided into several group of devices, with each group assigned to serve a specific subset of LLMs using intra-operator parallelism. The primary objective is to find the group of LLM bundles that maximizes the cluster utilization, i.e. the serving throughput. 

However, determining the optimal group of LLM bundles poses a challenging combinatorial optimization problem. As the number of devices and models increases, the total number of possible LLM bundle combinations grows exponentially. To solve this optimization problem, we design a two-level algorithm. As described in \Cref{alg:placement}, \Sys first enumerates potential device mesh groups. Each mesh comprises several GPUs that will be used to serve a set of LLMs concurrently. Then \Sys solves an ILP problem to find the best LLM bundles for a given device mesh group. \Sys selects the group of LLM bundles that achieve the highest estimated serving throughput as the serving configuration.


In \Cref{alg:placement}, \Sys needs to generate all possible model partition candidates to formulate the ILP problem. \Cref{alg:candidate} shows the pseudo-code to generate candidates. For each LLM, \Sys enumerates all possible configuration combinations of number of SMs and intra-operator parallelism degree. \Sys estimates throughput for each configuration, and selects the configuration that requires minimum number of SMs for each intra-operator parallelism degree as possible partition candidate. 

\textbf{Throughput Estimator.} Based on the observation that the serving throughput of LLMs is dominated by \textit{decoding} phases, we estimate the throughput by considering only \textit{decoding} phases. We begin by offline profiling the latency associated with different batch sizes and generation lengths. With the profiling results, we can then estimate the serving throughput and identify the minimum batch size that meets the requested arrival rate. 

\begin{algorithm}[t]
   \caption{Enumeration-based Model Placement}
   \label{alg:placement}
\begin{algorithmic}
   \STATE {\bfseries Input:} LLM list $M$, cluster $C$, workload $W$
   \STATE {\bfseries Output:} The group of LLM bundle $best\_bundles$
   \STATE $\mathcal{D} \leftarrow$ get\_potential\_device\_meshes($C$, $M$)
   \STATE $\hat{M} \leftarrow$ get\_partition\_candidate($M$, $W$)

   \STATE $best\_tpt, best\_bundles \leftarrow 0, None$
   \FOR{$D \in \mathcal{D}$}
   \STATE $bundles, tpt \leftarrow$ ILP\_bundle\_opt($\hat{M}$, $D$)
   \IF{$best\_tpt < tpt$}
   \STATE $best\_tpt, best\_bundles \leftarrow tpt, bundles$
   \ENDIF
   \ENDFOR
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
   \caption{Model Partition Candidate Generation}
   \label{alg:candidate}
\begin{algorithmic}
   \STATE {\bfseries Input:} LLM list $M$, workload $W$
   \STATE {\bfseries Output:} The parition candidate $\hat{M}$
   \STATE $\hat{M} \leftarrow []$
   \FOR{$m \in M$}
   \STATE $sm\_list \leftarrow$ get\_potential\_sm\_list($m$)
   \STATE $tp\_list \leftarrow$ get\_potential\_tp\_degree($m$)
   \STATE $model\_candidate \leftarrow \{\}$
   \FOR{$p \in tp\_list$}
   \FOR{$num\_sm \in$ sorted($sm\_list$)}
   \STATE $tpt, bs \leftarrow$ estimate\_throughput($m, num\_sm, p$)
   \IF{$tpt \ge W$.get\_rate($m$)}
   \STATE $model\_candidate$.add(($p, num\_sm, bs$))
   \STATE {\bfseries break}
   \ENDIF
   \ENDFOR
   \ENDFOR
   \STATE $\hat{M}$.append($model\_dandidate$)
   \ENDFOR
\end{algorithmic}
\end{algorithm}

\subsubsection{ILP formulation}

Given a device mesh group $D$ and a list of model partition candidates $\hat{M}$, \Sys formulates an ILP problem to find the group of LLM bundles that can maximize throughput. 

We define a one-hot decision vector $x \in \{0, 1\}^{|M|\times |D|}$ to represent the LLM bundles it created and $x_{i,j} = 1$ denotes that LLM $M_i$ and devich mesh $D_j$ are in the same LLM bundle. For each device mesh $D_j$, we use $a_{i,j}, b_{i, j}$ to denote the number of SMs and memory required to place LLM $M_i$ on it in order to achieve target serving throughput, respectively. The ILP problem should satisfy the following constraints,

\begin{equation}
\begin{aligned}
    \sum_{j} x_{i,j} &= 1 \\
    \sum_{i} a_{i,j} x_{i,j} &\le SM_{j}  \\
    \sum_{i} b_{i,j} x_{i,j} &\le MEMORY_{j} \\
\end{aligned}
\end{equation}

where $SM_{j}, MEMORY_{j}$ denote the the total number of SMs and size of memory of device mesh $D_j$. Given a fixed device mesh, the intra-operator parallelism degree of the LLMs to be placed on it is also determined. Therefore, $a_{i, j}$ and $b_{i, j}$ can be pre-computed as constants. The objective of the problem can be formulated as,
\begin{equation}
    \argmax_{x} \sum_{i,j} w_{i} \cdot p_{i,j} \cdot x_{i,j}
\end{equation}

where $p_{i,j}$ denotes the estimated throughput to place LLM $M_i$ on device mesh $D_j$, and $w_{i}$ represents the serving rate of LLM $M_i$. We use $w_{i}$ as a regulation term to enforce fair sharing among different LLMs. 

The constraints and objective are all linear, and we can solve it optimally with a solver. Once the decision vector $x$ is decided by ILP, we can get the best LLM bundle group in the device mesh group.
